A Robust Hierarchical Solver for Ill-conditioned Systems with Applications to Ice Sheet Modeling

A hierarchical solver is proposed for solving sparse ill-conditioned linear systems in parallel. The solver is based on a modification of the LoRaSp method, but employs a deferred-compression technique, which provably reduces the approximation error and significantly improves efficiency. Moreover, the deferred-compression technique introduces minimal overhead and does not affect parallelism. As a result, the new solver achieves linear computational complexity under mild assumptions and excellent parallel scalability. To demonstrate the performance of the new solver, we focus on applying it to solve sparse linear systems arising from ice sheet modeling. The strong anisotropic phenomena associated with the thin structure of ice sheets creates serious challenges for existing solvers. To address the anisotropy, we additionally developed a customized partitioning scheme for the solver, which captures the strong-coupling direction accurately. In general, the partitioning can be computed algebraically with existing software packages, and thus the new solver is generalizable for solving other sparse linear systems. Our results show that ice sheet problems of about 300 million degrees of freedom have been solved in just a few minutes using a thousand processors.

==> parallel.tex <==

\section{Parallel Algorithm} \label{CC:sec:parallel}

In this section, we present the parallel algorithm focusing on distributed-memory machines. Since data dependency is exactly the same as in the original LoRaSp method, the same parallel algorithm works here (with minor changes on what data is communicated). For sake of completeness, we briefly review the parallel algorithm in \cite{CC:chen2016parallel}.



